Large Language Models for Web Accessibility: A Systematic Literature Review

Web accessibility aims to ensure that web content and services are usable by people with diverse abilities. In recent years, Large Language Models (LLMs) have been increasingly explored to support accessibility-related tasks on the web, such as content generation, issue detection, and remediation. However, little is known about the characteristics of these approaches, the accessibility issues they target, the standards they follow, and how they are evaluated. In this paper, we present a systematic literature review of 38 peer-reviewed studies that investigate the use of LLMs in web accessibility contexts. We begin by performing a comprehensive search of scientific publications to identify relevant studies. We then conduct a comparative analysis to examine the accessibility tasks addressed, the LLM models and prompting strategies employed, the system architectures adopted, the accessibility issues and guidelines considered, and the evaluation methods used across studies. Our findings show that most studies apply LLMs to text-centric and structurally explicit accessibility tasks, with WCAG serving as the primary reference framework and limited consideration of cognitive accessibility guidelines (COGA). The reviewed approaches predominantly rely on general-purpose LLMs and prompt-based interactions, while evaluation practices vary widely and often lack direct involvement of users with disabilities. We envision this review as a consolidated reference for researchers and practitioners seeking to understand the current landscape of LLM-supported web accessibility, and as a foundation to guide future research and tool development in this area.

==> Sections/Background.tex <==
\section{Related Work}
\label{sec:RelatedWork}


==> Sections/Limitations.tex <==
\section{Limitations}
\label{sec:Limitations}

This section briefly discuss the limitations of our study. First, participants were selected by convenience and are mostly students enrolled in universities associated with the authors of this paper, which may decrease the profile diversity. Nevertheless, the demographic data shows participants with different backgrounds levels and experience in studying and applying usability concepts. 
Second, we evaluate the tool and its effect on theoretical and practical skills only based on participants perception as they filled out the survey applied after using the tool to learn the Nielsen's heuristics. Finally, the tool itself can be improved in many ways. We asked participants what they least enjoyed in our tool, and following is a summary of what they answered: confusing or unclear interface at some points, issues with UI Builder (e.g. resizing components, unclear instructions), repetitive or difficult quizzes, accessibility concerns, content delivery choices (e.g. lengthy texts readings, lack of examples), and lack of customization features.

==> Tables/disability.tex <==
\begin{table*}
\centering
\caption{Disability types studied across the reviewed papers (N=37).}
\vspace{-0.3cm}
\begin{adjustbox}{width=1.1\textwidth,center}
\begin{tabular}{|c|l|l|c|c|}
\hline
\rowcolor{gray!60}
\textbf{No.} &
\multicolumn{1}{c|}{\textbf{Type of Disability}} &
\multicolumn{1}{c|}{\textbf{PS}} &
\multicolumn{1}{c|}{\textbf{Count}} &
\multicolumn{1}{c|}{\textbf{Percentage (out of 37)}} \\
\hline

\textbf{01} & \textbf{Visual Impairment (Blind/Low Vision)} &
PS\#1, PS\#2, PS\#6, PS\#7, PS\#8, PS\#30, PS\#11, PS\#12, PS\#13, PS\#31, PS\#14, PS\#15, PS\#16, PS\#17, PS\#18, PS\#19, PS\#33, PS\#34, PS\#20, PS\#25, PS\#27, PS\#36 &
\textbf{22} & \textbf{59.46\%} \\
\hline

\rowcolor{gray!30}
\textbf{02} & \textbf{Cognitive / Learning / Intellectual Disability} &
PS\#1, PS\#3, PS\#30, PS\#26, PS\#27, PS\#29 &
\textbf{6} & \textbf{16.22\%} \\
\hline

\textbf{03} & \textbf{Motor / Physical Impairment} &
PS\#3, PS\#8, PS\#12, PS\#27 &
\textbf{4} & \textbf{10.81\%} \\
\hline

\rowcolor{gray!30}
\textbf{04} & \textbf{Deaf/Hard of Hearing} &
PS\#30, PS\#13, PS\#27, PS\#29 &
\textbf{4} & \textbf{10.81\%} \\
\hline

\textbf{05} & \textbf{General / Unspecified Disability} &
PS\#4, PS\#5, PS\#37, PS\#9, PS\#10, PS\#32, PS\#21, PS\#22, PS\#28, PS\#35 &
\textbf{10} & \textbf{27.03\%} \\
\hline

\rowcolor{gray!30}
\textbf{06} & \textbf{Not Reported} &
PS\#23, PS\#24 &
\textbf{2} & \textbf{5.41\%} \\
\hline

\end{tabular}
\end{adjustbox}
\label{tab:disability_types}
\end{table*}


==> Tables/llm_table.tex <==
\begin{table*}
\centering
\caption{Merged LLM families and the specific model variants reported in the reviewed papers.}
\vspace{-0.3cm}
\begin{adjustbox}{width=1.1\textwidth,center}
\begin{tabular}{|c|l|c|l|}
\hline
\rowcolor{gray!60}
\textbf{No.} & \multicolumn{1}{c|}{\textbf{LLM Name}} & \multicolumn{1}{c|}{\textbf{Count}} & \multicolumn{1}{c|}{\textbf{Models Included (Merged)}} \\ \hline

\textbf{01} & \textbf{GPT} & \textbf{20} & GPT-4o, GPT-4, GPT-4o mini, GPT-4V, GPT-4 Vision, GPT-3.5, GPT3.5 \\ \hline
\rowcolor{gray!30}
\textbf{02} & \textbf{ChatGPT} & \textbf{14} & ChatGPT, ChatGPT 3.5, ChatGP 3.5, ChatGPT 4.1, ChatGPT 4o, ChatGPT V4 \\ \hline
\textbf{03} & \textbf{Claude} & \textbf{7} & Claude 3.5 Sonnet, Claude 3.5 Haiku, Claude 3, Claude 2, Claude 3.7 Sonnet \\ \hline
\rowcolor{gray!30}
\textbf{04} & \textbf{Gemini} & \textbf{5} & Gemini, Gemini 1.5 Pro, Gemini 2.0 Flash \\ \hline
\textbf{05} & \textbf{LLaVA} & \textbf{3} & Video-LLaVA, LLaVA-NeXT-Video, LLaVA-OneVision \\ \hline
\rowcolor{gray!30}
\textbf{06} & \textbf{Llama} & \textbf{2} & Llama 3.1 \\ \hline
\textbf{07} & \textbf{DeepSeek} & \textbf{2} & DeepSeek, DeepSeek (V3) \\ \hline
\rowcolor{gray!30}
\textbf{08} & \textbf{Copilot} & \textbf{2} & Copilot, GitHub Copilot Pro \\ \hline
\textbf{09} & \textbf{Bard} & \textbf{2} & Google Bard, BARD \\ \hline
\rowcolor{gray!30}
\textbf{10} & \textbf{o3} & \textbf{2} & o3-mini \\ \hline
\textbf{11} & \textbf{FigmaAI} & \textbf{1} & FigmaAI \\ \hline
\rowcolor{gray!30}
\textbf{12} & \textbf{Galileo} & \textbf{1} & Galileo \\ \hline
\textbf{13} & \textbf{VILA} & \textbf{1} & VILA \\ \hline
\rowcolor{gray!30}
\textbf{14} & \textbf{Phi} & \textbf{1} & Phi 3 \\ \hline
\textbf{15} & \textbf{Gemma} & \textbf{1} & Gemma 2 \\ \hline
\rowcolor{gray!30}
\textbf{16} & \textbf{Mistral} & \textbf{1} & Mistral \\ \hline
\textbf{17} & \textbf{Grok} & \textbf{1} & Grok 3 \\ \hline
\rowcolor{gray!30}
\textbf{18} & \textbf{MiniGPT} & \textbf{1} & MiniGPT-4 \\ \hline

\end{tabular}
\end{adjustbox}
\label{tab:llm_merged_models}
\end{table*}


==> Tables/tools.tex <==
\begin{table*}
\centering
\caption{Tool types reported across the reviewed papers.}
\vspace{-0.3cm}
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{tabular}{|c|l|l|c|c|}
\hline
\rowcolor{gray!60}
\textbf{No.} &
\multicolumn{1}{c|}{\textbf{Tool Type}} &
\multicolumn{1}{c|}{\textbf{PS}} &
\multicolumn{1}{c|}{\textbf{Count}} &
\multicolumn{1}{c|}{\textbf{Percentage}} \\
\hline

\textbf{01} & \textbf{Automated Tool / Framework} &
PS\#2, PS\#37, PS\#30, PS\#12, PS\#15, PS\#16, PS\#17, PS\#18, PS\#34, Not Found, PS\#21, PS\#23, PS\#26, PS\#28, PS\#29 &
\textbf{15} & \textbf{34.10\%} \\
\hline

\rowcolor{gray!30}
\textbf{02} & \textbf{Browser Extension} &
PS\#7, PS\#31, PS\#33, PS\#20, PS\#25 &
\textbf{5} & \textbf{11.40\%} \\
\hline

\textbf{03} & \textbf{Dataset / Benchmark} &
PS\#22 &
\textbf{1} & \textbf{2.30\%} \\
\hline

\rowcolor{gray!30}
\textbf{04} & \textbf{Hybrid Approach / Workflow} &
PS\#1, PS\#3, PS\#35 &
\textbf{3} & \textbf{6.80\%} \\
\hline

\textbf{05} & \textbf{LLM Agent / Assistant} &
PS\#10, PS\#14, PS\#24 &
\textbf{3} & \textbf{6.80\%} \\
\hline

\rowcolor{gray!30}
\textbf{06} & \textbf{Application} &
PS\#36 &
\textbf{1} & \textbf{2.30\%} \\
\hline

\textbf{07} & \textbf{Prompt Engineering Strategy} &
PS\#4, PS\#5, PS\#8, PS\#9, PS\#11, PS\#13, PS\#32, PS\#19, PS\#27 &
\textbf{9} & \textbf{20.50\%} \\
\hline

\rowcolor{gray!30}
\textbf{08} & \textbf{Recommendations / Guidelines} &
PS\#6 &
\textbf{1} & \textbf{2.30\%} \\
\hline

\hline

\end{tabular}
\end{adjustbox}
\label{tab:tool_types}
\end{table*}




